Distributionally Robust Lyapunov Function Search Under Uncertainty

This paper develops methods for proving Lyapunov stability of dynamical systems subject to disturbances with an unknown distribution. We assume only a finite set of disturbance samples is available and that the true online disturbance realization may be drawn from a different distribution than the given samples. We formulate an optimization problem to search for a sum-of-squares (SOS) Lyapunov function and introduce a distributionally robust version of the Lyapunov function derivative constraint. We show that this constraint may be reformulated as several SOS constraints, ensuring that the search for a Lyapunov function remains in the class of SOS polynomial optimization problems. For general systems, we provide a distributionally robust chance-constrained formulation for neural network Lyapunov function search. Simulations demonstrate the validity and efficiency of either formulation on non-linear uncertain dynamical systems.

==> computation-graph.tex <==
\begin{tikzpicture}
\providecommand{\bfx}{\mathbf{x}}
\providecommand{\Lie}{\mathcal{L}}
\providecommand{\grad}{\nabla}
\providecommand{\GP}{GP}
\providecommand{\ubfu}{\underline{\mathbf{u}}}
\node [] (gh) {$\grad_\bfx h(\bfx)$};

\node [right=of gh] (L1) {$\underbrace{\grad_\bfx h(\bfx)^\top f(\bfx)}_{\Lie_f h(\bfx)}$};

\path [->,color=red] (gh)  edge [above] node {$[\cdot]$} (L1);

\node [below=of L1] (f1) {$f(\bfx) \sim \GP $};

\path [->,color=red] (f1)  edge [left] node {$[\cdot]$} (L1);

\node [right=of L1] (gL1) {$\grad_\bfx \Lie_f h(\bfx)$};

\path [->,color=blue] (L1)  edge [above] node {$\grad_\bfx$} (gL1);

\node [right=of gL1] (L2) {$\grad_\bfx[\Lie_f h(\bfx)]^\top F(\bfx) \ubfu$};

\node [below=38pt of L2] (f2) {$F(\bfx)\ubfu \sim \GP $};

\path [->,color=red] 
(f2) edge 
    node[above] {$[\cdot]$}
    node[below] {$\ubfu = [1, \mathbf{0}^\top_m]^\top$} 
 (f1);

\path [->,color=red] (f2)  edge [left] node {$[\cdot]$} (L2);

\path [->,color=red] (gL1)  edge [above] node {$[\cdot]$} (L2);

%\node [right=of L2] (gL2) {};
%\draw[dotted] (L2) -- (gL2) ;
%\path[clip] (gh.north west) rectangle (f2.south east); 
\end{tikzpicture}



==> tex/CLF_SOS.tex <==
\section{Distribuionally Robust CLF Search via Sum of Squares}
\label{sec: sos_clf}

%link: https://bcci.me.berkeley.edu/downloads/papers/weehong_3.pdf


Inspired by the formulations in \eqref{eq: original_clf_sos}, given a polynomial nominal controller $\beta(\bfx)$, we now consider the distributionally robust formulation as follows, 
%
\begin{equation}
\label{eq: drccp_clf_sos}
    \inf_{\mathbb{P}\in \calM_{N}^{r}}\bbP(-\dot{V}(\bfx,\bfxi) - \epsilon\|\bfx\|_2^2 \geq 0  ) \geq 1-\alpha \; \forall \bfx \in \calX ,
\end{equation}
%
We first write down the expression for $\dot{V}(\bfx,\bfxi)$ with model uncertainty in \eqref{eq: uncertain_control_affine}. Using the kronecker product property $\text{vec}(\bfA\bfB\bfC) = (\bfC^\top \otimes \bfA)\text{vec}(\bfB)$ and the vectorization of $F(\bfx)$ in \eqref{eq: F_vectorization}, we have
%
\begin{align}
\label{eq: V_dot_control_affine}
    &\dot{V}(\bfx,\bfxi) = [\nabla_{\bfx} V(\bfx)]^\top F(\bfx)\beta(\bfx) + aV(\bfx) \notag \\
     &= \beta(\bfx)^\top \text{vec}([\nabla_{\bfx} V(\bfx)]^\top F(\bfx)\bfI_{m+1}) + aV(\bfx) \notag \\
    &= \beta(\bfx)^\top(\bfI_{m+1} \otimes [\nabla_{\bfx} V(\bfx)]^\top)\text{vec}(F(\bfx)) + aV(\bfx) \notag \\
    % &= \beta(\bfx)^\top(\bfI_{m+1} \otimes [\nabla_{\bfx} V(\bfx)]^\top)\text{vec}(\tilde{F}(\bfx)+\sum_{i=1}^k W_i(\bfx)\xi_i) + \alpha_V(V(\bfx)) \notag \\
    & = \beta(\bfx)^\top \underbrace{(\bfI_{m+1} \otimes [\nabla_{\bfx} V(\bfx)]^\top)\text{vec}(\tilde{F}(\bfx))}_{q(\bfx)}+ aV(\bfx) + \notag \\
    & \;\; \beta(\bfx)^\top \underbrace{(\bfI_{m+1} \otimes [\nabla_{\bfx} V(\bfx)]^\top) \bfW(\bfx)}_{\bfR(\bfx)} \bfxi \notag \\
    & = \beta(\bfx)^\top q(\bfx) + \beta(\bfx)^\top \bfR(\bfx) \bfxi + aV(\bfx).
\end{align}
%
We now have the function $\dot{V}(\bfx, \bfxi)$ is affine in the uncertainty $\bfxi$. Following the same technique as in Proposition~\ref{proposition: drcc_sos}, we develop the distributionally robust chance constrained formulation of searching for a control Lyapunov function for the uncertain dynamical system \eqref{eq: uncertain_control_affine} as follows, 
%
\begin{align}
\label{eq: drccp_sos_clf_final}
    &V(\bfx) = \sum_{i=1}^{d} c_i \bfx^i, \; c_0 = 0, \notag \\
     &V(\bfx) - \epsilon\|\bfx\|_2^2 \in \text{SOS}(\bfx); \notag \\
    - & r \beta(\bfx)^\top \bfR(\bfx)_j - \alpha(\dot{V}(\bfx,\bfxi_i) - \epsilon\|\bfx\|_2^2) \in \text{SOS}(\bfx), \notag \\
    &r \beta(\bfx)^\top \bfR(\bfx)_j - \alpha(\dot{V}(\bfx,\bfxi_i) - \epsilon\|\bfx\|_2^2) \in \text{SOS}(\bfx), \notag \\
    & \forall i = 1,2 \dots, N, \quad \forall j = 1,2 \dots, k. 
\end{align}





% where $\bfx \in \calX \subseteq \mathbb{R}^{n}$ is the robot state and $\bfu \in \mathcal{U} \subseteq \mathbb{R}^{m}$ is the control input.  We assume $f : \mathbb{R}^{n} \mapsto \mathbb{R}^{n}$ and $g : \mathbb{R}^{n} \mapsto \mathbb{R}^{n \times m}$ are continuously differentiable.
% The admissible control input space is given by $\calU \coloneqq \{\bfu \in \mathbb{R}^m \,|\, A \bfu \leq \boldsymbol{b} \}$, where $A \in \mathbb{R}^{k \times m}$ and $\boldsymbol{b} \in \mathbb{R}^k$.
% suppose that $f(\bf0) = 0$. A function $V$ is a Control Lyapunov Function (CLF) for this system if $V: \mathbb{R}^n \mapsto \mathbb{R}_{\geq 0}$ is a
% smooth, radially unbounded function such that: 
% \begin{equation}
% \label{eq: CLF_Origin}
%     \inf_{\bfu \in \mathbb{R}^m} \{ \frac{\partial V}{\partial \bfx} f(\bfx) + \frac{\partial V}{\partial \bfx} g(\bfx)\bfu\} < 0.
% \end{equation}
% Note that for any $\bfx \in \calX$ such that $\frac{\partial V}{\partial \bfx} g(\bfx) \neq 0$, one can make the inequality hold in \eqref{eq: CLF_Origin} by choosing a large value of $\bfu$ of the correct sign (requires no restriction on control space). Thus, the critical part is to satisfy the following condition:
% %
% \begin{equation}
%     \frac{\partial V}{\partial \bfx} f(\bfx) < 0 \; \; \forall \bfx \in \calX \; \text{such that} \; \frac{\partial V}{\partial \bfx} g(\bfx) = 0, \bfx \neq \bf0.
% \end{equation}
% \TODO{If we restrict $f$ and $g$ be polynomial vector fields}, we can use SOS programming
% to search for a polynomial CLF $V$.

% The problem now becomes: 
% \begin{align}
% \label{eq:origin_search}
%     &\text{find} \; V \in \calR_n \quad \quad \text{such that} \\
%     & V(\bfx) > 0 \; \forall \bfx \in \mathbb{R}^n \backslash \boldsymbol{0}, \; V(\boldsymbol{0}) = 0 \notag \\
%     & \Big\{ \bfx \in \mathbb{R}^n |  \frac{\partial V}{\partial \bfx} g(\bfx) = 0,   \frac{\partial V}{\partial \bfx} f(\bfx) \geq 0, \bfx \neq \bf0  \Big\} \text{is empty} \notag
% \end{align}

% \TODO{Based on the Positivstellensatz (P-satz), it is shown that the following SOS optimization program is a sufficient condition for problem \eqref{eq:origin_search} :} 
% %
% \begin{align}
% \label{eq: sos_clf}
%   &\min \gamma \quad \quad \text{over} \quad s_1 \in \Sigma_n,\; V,p_2 \in \calR_n \; \text{such that} \notag \\
%   & V-l_1 \in \Sigma_n; \notag \\
%   & -\Big\{ s_1 \left[ \frac{\partial V}{\partial \bfx} f(\bfx) - \gamma \right] + p_2 \left[\frac{\partial V}{\partial \bfx} g(\bfx) \right] \Big\} - l_2 \in \Sigma_n.
% \end{align}
% %
% where $\calR_n$ denotes the set of all polynomials of $n$ variables, $\Sigma_n$ denotes the set of sum of squares polynomials in $n$ variables, and $l_1, l_2$ are positive definite SOS polynomials. To ensure that \eqref{eq: sos_clf} has a chance of being satisfied, the polynomials we are searching over must satisfy the following degree conditions:
% %\KL{Why the degree conditions?}
% %
% \begin{align}
%     &\text{deg} V = \text{deg} l_1; \\
%     &\text{deg}(p_2Vg) \geq \text{deg} (s_1 V f); \\
%     &\text{deg} (p_2Vg) - 1 = \text{deg} l_2
% \end{align}
% %
% Note that the second constraint is binlinear (non-convex), the authors use iterative searching method to find the solution. 

% Furthermore, if we assume that the system is uncertain
% %
% \begin{equation}
%     \dot{\bfx} = f(\bfx)+g(\bfx)\bfu + d(\bfx)\bfomega, \; \bfomega \in \Omega
% \end{equation}
% %
% where
% %
% \begin{equation}
%     \Omega = \{ \bfomega \in \mathbb{R}^k: k_{\omega_i}(\bfomega) \geq 0, i = 1, \cdots, n_{\omega} \}
% \end{equation}
% %
% We can reformulate the SOS program in \eqref{eq: sos_clf} as follows: 
% %
% \begin{align}
%     &\min \gamma \quad \quad \text{over} \quad s_1 \in \Sigma_n,\; V,p_2 \in \calR_n \; \text{such that} \notag \\
%   & V-l_1 \in \Sigma_n; \notag \\
%   & -\Big\{ s_1 \left[ \frac{\partial V}{\partial \bfx} f(\bfx) - \gamma \right] + p_2 \left[\frac{\partial V}{\partial \bfx} g(\bfx) \right] +l_2  + \notag \\ &\sum_{i=1}^{n_\omega} \alpha_i(\bfx,\omega) k_{\omega_i}(\omega)\Big\} \in \text{SOS}(\bfx,\omega); \notag \\
%   &\alpha_i(\bfx,\omega) \in \text{SOS}(\bfx,\omega).
% \end{align}
% %
% where $l_1 = l_2 = \epsilon\|\bfx\|_2^2$. 






% Another way of adding uncertainty in the SOS formulation is that, for any $\bfx \in \calX$, 
% %
% \begin{align}
%     &-\mathbb{E}[\dot{V}(\bfx,\omega)] \geq \epsilon \|\bfx\|_2^2 \\
%     &-\text{CVaR}_{\beta}[\dot{V}(\bfx,\omega)] \geq \epsilon \|\bfx\|_2^2 \\
%     & \inf_{\mathbb{P} \in \calM}\mathbb{P} (-\dot{V}(\bfx,\omega)  \geq \epsilon \|\bfx\|_2^2) \geq 1 - \alpha
% \end{align}
%





 




































==> tex/CLF_Search.tex <==
\section{Control Lyapunov Function Search For Open-loop Systems with Model Uncertainty}
\label{sec: clf_nn_search}

In this section, we present an learning-based approach for solving Problem.~\ref{prob: CLF_Construction}. The SOS technique is restricted to polynomial systems and it is generally hard to find SOS CLFs with  controllers simultaneously, even for known non-linear control-affine systems \cite{TanSearchingFC, jarvis_clf_sos}. This motivates us to consider a data-driven approach, similar to Sec.~\ref{sec: nn_lf_search}. 

Inspired by the recent advances in learning neural network certificates for control \cite{Dawson_2022_survey, dai_2021_lyapunov, dawson_2022_robust_CLBF, Chang2019NeuralLC}, we consider applying the distributionally robust formulation to search for a neural network CLF. Once a distributionally robust chance constrained neural network CLF (DRCC-NN-CLF) is found, we utilize the CLF-QP \eqref{eq: clf_qp} to synthesize stable controllers online for uncertain control-affine systems in \eqref{eq: uncertain_control_affine}. 
 
% \subsection{Neural Network Lyapunov Function and Controller}
% \textcolor{blue}{Since the global condition (SOS) for Lyapunov function is hard to impose, we can consider the data-driven (neural nets) approach, where we impose the chance-constrained condition for all the discretization points over $\bbR^n$. }
We consider a neural network representation of CLF $V_{\bftheta} = \phi_{\bftheta}(\bfx)^\top \phi_{\bftheta}(\bfx)$, where $\phi_{\bftheta}$ is a fully-connected neural network with parameter $\bftheta$. In the offline training stage, our goal is to construct a CLF $V_{\bftheta}(\bfx)$ such that the conditions in \eqref{eq: clf_conditions} are satisfied in the domain of interest. Similar to Sec.~\ref{sec: nn_lf_search}, the training set $\calD_{\text{CLF}} := \{ \bfx_i\}_{i=1}^M$ is constructed by sampling $\{ \bfx_i\}_{i=1}^M$ uniformly from the domain of interest $\calX$; we also have the uncertainty training set $\calD_{\xi} := \{ \bfxi_i\}_{i=1}^N$. We aim at searching a DRCC-NN-CLF $V_{\bftheta}$ for the general uncertain control-affine system \eqref{eq: uncertain_control_affine} and use the learned $V_{\bftheta}$ to synthesize stable controllers online, even for online uncertainty $\bfxi^{*}$ that may from a different distribution $\bbP^{*}$ other than $\bbP$.

We denote the control Lyapunov condition (CLC) as, (In the following discussions, we write $V(\bfx)$ to denote the neural network representation $V_{\bftheta}(\bfx)$)
%
\begin{align}
\label{eq: clc_def}
    \textit{CLC}(\bfx,\ubfu) &:= \mathcal{L}_f V(\bfx) + \mathcal{L}_g V(\bfx)\bfu + \alpha( V(\bfx))
    = [\nabla_{\bfx} V(\bfx)]^\top F(\bfx)\ubfu + \alpha(V(\bfx)).
\end{align}
%
% Inspired by our discussions in Sec.~\ref{sec: drccp_lf}, we consider the distributionally robust chance-constraint formulation of \eqref{eq: relaxed_clf_qp},
Note that the positive definiteness of $V_{\bftheta}$ is preserved by construction. Inspired by \cite{Dawson_2022_survey}, we consider the following empirical loss for training a candidate DRCC-NN-CLF $V_{\bftheta}$,
%
\begin{equation}
\label{eq: CLF_loss}
    \ell_{\text{DR-CLF}}(\bftheta) = \lambda_1 V_{\bftheta}(\boldsymbol{0})
     + \frac{\lambda_2}{M}\sum_{i=1}^M \delta(\bfx_i)
\end{equation}
%
where $[\delta(\bfx_i), \bfu_i]$ are the solutions to the following relaxed distributionally robust version of CLF-QP \eqref{eq: clf_qp} at each state $\bfx_i$,
%
% \begin{equation}
% \begin{aligned}
% \label{eq: relaxed_clf_qp}
%     &\min_{\bfu \in \calU, \delta \in \bbR} \| \bfu\|^2 + \lambda_3 \delta,  \\
%     \mathrm{s.t.} \, \, &L_f V(\bfx) + L_g V(\bfx)\bfu + \alpha( V(\bfx)) \leq \delta, \; \; \delta \geq 0.
% \end{aligned}
% \end{equation}
%
\begin{equation}
\begin{aligned}
\label{eq: drccp_clf_qp}
    &\min_{\ubfu \in \underline{\calU}, \delta \in \bbR} \| \ubfu\|^2 + \lambda_3 \delta,  \\
    \mathrm{s.t.} \, \, & \inf_{\mathbb{P} \in \calM_{N}^{r}}\bbP(\textit{CLC}(\bfx, \ubfu, \bfxi) \leq \delta) \geq 1 - \beta, \; \; \delta \geq 0.
\end{aligned}
\end{equation}
%
Note that $\delta$ can be back-propagated as a layer to the original network architecture \cite{cvxpylayers2019} if the program \eqref{eq: drccp_clf_qp} is convex. In the following, we propose our approach that formulates \eqref{eq: drccp_clf_qp} as a tractable quadratic program (QP). 

% If dealing with a general uncertain control-affine system \eqref{eq: uncertain_control_affine}, where $f$ and $g$ are not perfectly known, one should consider taking the uncertainty into account for the constraint in \eqref{eq: relaxed_clf_qp}. We denote the control Lyapunov condition (CLC) as, 
%
% \begin{align}
% \label{eq: clc_def}
%     \textit{CLC}(\bfx,\ubfu) &:= \mathcal{L}_f V(\bfx) + \mathcal{L}_g V(\bfx)\bfu + \alpha( V(\bfx))
%     = [\nabla_{\bfx} V(\bfx)]^\top F(\bfx)\ubfu + \alpha(V(\bfx))
% \end{align}
%

% Specifically, for chance-constrained formulation, we consider
% %
% \begin{equation}
% \begin{aligned}
% \label{eq: ccp_clf_qp}
%     &\min_{\bfu \in \calU, r \in \bbR} \| \bfu\|^2 + \lambda_5 \delta,  \\
%     \mathrm{s.t.} \, \, & \bbP(\textit{CLC}(\bfx, \ubfu, \bfxi) \leq \delta) \geq 1 - \beta, \\
%     & \delta \geq 0.
% \end{aligned}
% \end{equation}
% %
% where $\beta$ denotes some user-specified risk tolerance. As shown in Proposition.~\ref{proposition: convex_remove_inf}, if we pick $\beta \leq \frac{1}{N}$, one can relax \eqref{eq: ccp_clf_qp} as the following program 
% %
% \begin{equation}
% \begin{aligned}
% \label{eq: relaxed_ccp_clf_qp}
%     &\min_{\bfu \in \calU, r \in \bbR} \| \bfu\|^2 + \lambda_5 \delta,  \\
%     \mathrm{s.t.} \, \, & \max_i \textit{CLC}(\bfx, \ubfu, \bfxi_i) \leq \delta, \\
%     & \delta \geq 0.
% \end{aligned}
% \end{equation}
%
% namely, 
%
% \begin{equation}
% \begin{aligned}
% \label{eq: drccp_clf_qp}
%     &\min_{\ubfu \in \underline{\calU}, \delta \in \bbR} \| \ubfu\|^2 + \lambda_3 \delta,  \\
%     \mathrm{s.t.} \, \, & \inf_{\mathbb{P} \in \calM_{N}^{r}}\bbP(\textit{CLC}(\bfx, \ubfu, \bfxi) \leq \delta) \geq 1 - \beta, \; \; \delta \geq 0.
% \end{aligned}
% \end{equation}
%
We first write down the expression for CLC, using the nominal dyanmics $\tilde{F}$, perturbation matrix $\bfW(\bfx)$ and uncertainty $\bfxi$. By the kronecker product property $\text{vec}(\bfA\bfB\bfC) = (\bfC^\top \otimes \bfA)\text{vec}(\bfB)$ and the vectorization of $F(\bfx)$ in \eqref{eq: F_vectorization}, we have
%
\begin{align}
\label{eq: cLc_kronecker}
    &\textit{CLC}(\bfx,\ubfu,\bfxi) = [\nabla_{\bfx} V(\bfx)]^\top F(\bfx)\ubfu + \alpha(V(\bfx)) 
     = \ubfu^\top \text{vec}([\nabla_{\bfx} V(\bfx)]^\top F(\bfx)\bfI_{m+1}) +\alpha(V(\bfx)) \notag \\
    &= \ubfu^\top(\bfI_{m+1} \otimes [\nabla_{\bfx} V(\bfx)]^\top)\text{vec}(F(\bfx)) + \alpha(V(\bfx)) \notag \\
    % &= \ubfu^\top(\bfI_{m+1} \otimes [\nabla_{\bfx} V(\bfx)]^\top)\text{vec}(\tilde{F}(\bfx)+\sum_{i=1}^k W_i(\bfx)\xi_i) + \alpha(V(\bfx)) \notag \\
    & = \ubfu^\top\underbrace{(\bfI_{m+1} \otimes [\nabla_{\bfx} V(\bfx)]^\top)\text{vec}(\tilde{F}(\bfx))}_{q(\bfx)}+ \alpha(V(\bfx)) + \ubfu^\top \underbrace{(\bfI_{m+1} \otimes [\nabla_{\bfx} V(\bfx)]^\top) \bfW(\bfx)}_{\bfR(\bfx)} \bfxi \notag \\
    & = \ubfu^\top q(\bfx) + \ubfu^\top \bfR(\bfx) \bfxi +\alpha(V(\bfx)). 
\end{align}
%
Thus, $\textit{CLC}(\bfx,\ubfu, \bfxi)$ is affine in the uncertainty $\bfxi \in \mathbb{R}^{k}$ since $\tilde{F}(\bfx)$, $V(\bfx)$ and $\bfW(\bfx)$ are assumed to be deterministic. By the CVaR approximation of DRCC \eqref{eq: drccp_cvar_approximate}, we write 
%
\begin{align}
\label{eq: clf_qp_cvar}
& \min_{\ubfu \in \underline{\calU}, \delta \in \bbR_{\geq 0}}\,\, \|\ubfu\|^2 + \lambda_3 \delta, \\
% \bfu^T H \bfu + p_d \delta^2 \\
\mathrm{s.t.} \, \,  &\sup_{\mathbb{P}\in \calM_{N}^{r}}\inf_{t \in \mathbb{R}}[\beta^{-1}\mathbb{E}_{\bbP}[(\textit{CLC}(\bfx, \ubfu, \bfxi) - \delta +t  )_{+}] -t]  \leq  0, \notag
\end{align}
%
where the feasible set of \eqref{eq: clf_qp_cvar} is a subset of the feasible set of \eqref{eq: drccp_clf_qp}. Similar to our previous work~\cite[Proposition IV.1]{long2022_clf_cbf_drccp}, we propose a tractable reformulation to \eqref{eq: clf_qp_cvar}.

\begin{lemma}
\label{lemma: neural_net_drccp_qp}
Given the expression of $\textit{CLC}$ in \eqref{eq: cLc_kronecker} and suppose $\Xi = \bbR^k$. Consider the $1$-Wasserstein distance with metric $d$ being the $L_1$ norm, the following QP is equivalent to \eqref{eq: clf_qp_cvar},
\begin{align}
\label{eq: clf_qp_unbounded_final}
& \min_{\ubfu \in \underline{\calU}, \delta \in \bbR_{\geq 0}, t \in \bbR, s_i \in \bbR} \,\, \|\ubfu\|^2 + \lambda_3 \delta \qquad  \\
\mathrm{s.t.} \, \, 
& r |\ubfu^\top \bfR(\bfx) | \leq (t \beta - \frac{1}{N} \sum_{i=1}^{N} s_i) \mathbf{1}_{k}, \; \; s_i \geq 0, \notag \\
& s_i \geq \ubfu^\top q(\bfx) + t - \delta + \ubfu^\top \bfR(\bfx) \bfxi_i + \alpha(V(\bfx)) , \; \; \forall i \in [N]. \notag 
\end{align} 
\end{lemma}



% \begin{remark}
% {\rm Suppose that $\Xi = \{\bfxi \in \mathbb{R}^k \;|\; \bfC \bfxi \leq \bfd\}$ be compact, where $\bfC \in \mathbb{R}^{q \times k}$ and $\bfd \in \mathbb{R}^q$ for some $q > 0$. and the following optimization program is equivalent to \eqref{eq: clf_qp_cvar},
% \begin{align}
% \label{eq: clf_qp_final}
% & \min_{\ubfu \in \underline{\calU}, \delta \in \bbR_{\geq 0}, t \in \bbR, s_i \in \bbR, \zeta \in \bbR_{\geq 0}, \eta_{i} \in \bbR^q} \,\, \|\ubfu\|^2 + \lambda_3 \delta \qquad  \\
% \mathrm{s.t.} \, \, 
% & \zeta r + \frac{1}{N}\sum_{i=1}^N s_i - t\beta \leq 0, \; \; s_i \geq 0, \notag \\
% & s_i \geq \ubfu^\top q(\bfx) + t - \delta + (\ubfu^\top \bfR(\bfx) - \eta_{i}^\top \bfC) \bfxi_i + \eta_{i}^\top \bfd + \alpha(V(\bfx)) , \notag \\
% & |\ubfu^\top \bfR(\bfx) - \eta_{i}^\top \bfC | \leq \beta \mathbf{1}_{k}, \; \; \eta_{i} \geq \boldsymbol{0}, \; \; \forall i \in [N].  \notag
% \end{align}
% \hfill $\bullet$
% }
% \end{remark}

We compute the solutions of \eqref{eq: clf_qp_unbounded_final} during the training phase and use it in the loss function \eqref{eq: CLF_loss} for learning a candidate DRCC-NN-CLF. Then, for the uncertain control-affine system \eqref{eq: uncertain_control_affine}, we use the learned candidate CLF $V_{\bftheta}$ to synthesize a controller by solving a CLF-QP \eqref{eq: clf_qp} online. We observe that the stability of the closed-loop system with the controller solved by CLF-QP can be assured with high probability. 

% In the following, we show that the learned candidate CLF $V_{\bftheta}$ with distributionally robust loss function design in \eqref{eq: clf_qp_final} guarantees the stability of the closed-loop system with controllers solved by CLF-QP online with high probability, even for shifted system dynamics uncertainty. 

% \begin{proposition}
% \label{proposition: dr_nn_clf_guarantee}
% Suppose the loss function \eqref{eq: CLF_loss} goes to zero after training for sufficiently enough epochs, meaning that $\delta(\bfx_i) = 0$ for any $\bfx_i \in \calD_{\text{CLF}}$ with the learned $V_{\bftheta}$. Let the online uncertainty $\bfxi^{*}$ be drawn from some distribution $\bbP^{*} \in \calM_{N}^r$, then the stability of the closed-loop system with controllers solved by CLF-QP can be assured with probability greater than $1-\beta$. 

% \begin{proof}
% We first write 
% %
% \begin{equation}
% \label{eq: write_clc_as_r}
%     r(\bfx, \bbP) := \bbP(\textit{CLC}(\bfx, \ubfu(\bfx), \bfxi) \leq 0),
% \end{equation}
% %
% given that $\delta(\bfx_i) = 0$ for any $\bfx_i \in \calD_{\text{CLF}}$ with $V_{\bftheta}$, we know that there exists $\ubfu \in \underline{\calU}$ such that 
% \begin{equation*}
% \label{eq: stable_pf_1}
%     \forall \bfx_i \in \calD_{\text{CLF}}, \quad \inf_{\mathbb{P} \in \calM_{N}^{r}}\bbP(\textit{CLC}(\bfx_i, \ubfu, \bfxi) \leq 0) \geq 1 - \beta.
% \end{equation*}
% %
% Then, for any online uncertainty $\bfxi^*$ sampling from a distribution $\bbP^{*} \in \calM_N^r$, there exists $\ubfu_{*} \in \underline{\calU}$ such that
% \begin{equation*}
% \label{eq: stable_pf_2}
%     \forall \bfx_i \in \calD_{\text{CLF}}, \quad r(\bfx_i, \bbP^{*}) = \bbP^{*}(\textit{CLC}(\bfx_i, \ubfu_{*}, \bfxi^{*}) \leq 0) \geq 1 - \beta.
% \end{equation*}
% %
% Next, during the test time, for any $\bfx^* \in \calX$ and $\bfx^{*} \notin \calD_{\text{CLF}}$, our goal is to show that $r(\bfx^*, \bbP^*) \geq 1 - \beta$. 

% %



% \TODO{Complete the proof to show stability guarantees for any $\bfx^* \in \calX$ by using the Lipschitz property of system dynamics. Suppose $d(\bfx^*, \calD_{\text{CLF}}) <  \beta$, we need to show $r(\bfx, \bbP)$ is Lipschitz in the variable $\bfx$ with some constant $L$. Then, a sufficiently small $\beta$ guarantees a small change in the value of $r(\bfx, \bbP)$, thus the stability property with high probability is preserved. 

% Besides, could we modify the loss function (36) a bit by taking the Lipschitz constant into account? (i.e. a bit more conservative, $\bbP(\text{CLC}(\bfx, \ubfu, \bfxi) \leq \delta) \geq 1 - \beta + \hat{\beta}$? where $\hat{\beta}$ depends on $\beta$ and $L$.)}


% This implies that the closed loop system with the solved CLF-QP controller $\ubfu_{*}(\bfx)$ is point-wise stable with high probability.



% \end{proof}

% \end{proposition}



% \textcolor{blue}{We might be able to combine the chance constrained formulation into \eqref{eq:lyapunov_condition}. Specifically, $\mathbb{P} (\dot{V}_{\bftheta}(\bfx,\bfxi) \leq 0) \geq 1 - \beta$ can be approximated (with CVaR) by 
% $\frac{1}{N} \sum_{i=1}^{k} (\dot{V}_{\bftheta}(\bfx,\bfxi_i) - \dot{V}_{\bftheta}(\bfx,\bfxi_k)) + \beta (\dot{V}_{\bftheta}(\bfx,\bfxi_k)) \leq 0.$ }

% We can define the loss function as $\ell(\bftheta) := \ell_1(\bftheta) + \lambda \ell_2(\bftheta)$, with a parameter $\lambda > 0$ and:
% \begin{equation}
% \label{eq: loss_ccp}
% \begin{aligned}
% \ell_1(\bftheta) &:= \frac{1}{M}\sum_{i=1}^M (\max(0, -V_{\bftheta}(\bfx_i)) + V_{\bftheta}^2(\boldsymbol{0}),\\
% \ell_2(\bftheta) &:=  \frac{1}{M}\sum_{i=1}^M (\max(0, \frac{1}{N} \sum_{j=1}^{k} (\dot{V}_{\bftheta}(\bfx_i,\bfxi_j) - \dot{V}_{\bftheta}(\bfx_i,\bfxi_k)) 
%      \\
%      &+ \beta (\dot{V}_{\bftheta}(\bfx_i,\bfxi_j)))
% \end{aligned}
% \end{equation}

% \subsection{Control-Affine System}
% Consider the control-affine system,
% %
% \begin{equation}\label{eq: dynamic}
% \dot{\bfx} = f(\bfx)+g(\bfx)\bfu
% \end{equation}
% %
% and the uncertain control-affine system,
% %
% \begin{equation}\label{eq: uncertain_dynamic}
% \dot{\bfx} = f(\bfx)+g(\bfx)\bfu + d(\bfx)\bfxi
% \end{equation}
% %
% where $\bfx \in \calX \subseteq \mathbb{R}^{n}$ is the robot state and $\bfu \in \mathbb{R}^{m}$ is the control input. We assume $f : \mathbb{R}^{n} \mapsto \mathbb{R}^{n}$, $g : \mathbb{R}^{n} \mapsto \mathbb{R}^{n \times m}$ and $d: \mathbb{R}^{n} \mapsto \mathbb{R}^{n \times k}$ are continuously differentiable. 

% \textcolor{blue}{We start with only considering uncertainty in $f$.}


% \begin{definition}
% A continuously differentiable function $V: \mathbb{R}^n \mapsto {\mathbb{R}_{\geq 0}}$ is a \emph{control Lyapunov function (CLF)} for the system \eqref{eq: dynamic} if there exists a class $\mathcal{K}$ function $\alpha$ such that:
% %
% \begin{equation}
%     \inf_{\ubfu \in \underline{\mathcal{U}}} \textit{CLC}(\bfx,\ubfu) \leq 0, \quad \forall \bfx \in \calX,
% \end{equation}
% %
% where the \emph{control Lyapunov condition (CLC)} is:
% %
% \begin{equation}\label{eq:clc_define}
% \begin{aligned}
%     \textit{CLC}(\bfx,\ubfu) \delequal \mathcal{L}_f V(\bfx) + \mathcal{L}_g V(\bfx)\bfu + \alpha( V(\bfx)) 
%     %& = [\nabla_{\bfx} V(\bfx)]^\top f(\bfx) + [\nabla_{\bfx} V(\bfx)]^\top g(\bfx)\bfu + \alpha(V(\bfx)) \\ 
%     % & =  [\nabla_{\bfx} V(\bfx)]^\top F(\bfx)\ubfu + \alpha(V(\bfx)).
% \end{aligned}
% \end{equation}
% \end{definition}
% %
% One can consider the CLF-QP for stable control synthesis, 
% %
% \begin{equation}\label{eq:CLF_QP}
% \begin{aligned}
% & \min_{\ubfu \in \underline{\calU}}\,\, \|L(\bfx)^\top(\ubfu - \underline{\tilde{\bfk}}(\bfx))\|^2 \\
% % \boldsymbol{u}^T H \boldsymbol{u} + p_d \delta^2 \\
% \mathrm{s.t.} \, \,  &\textit{CLC}(\bfx,\ubfu) \leq 0. 
% \end{aligned}
% \end{equation}
% %
% \textcolor{blue}{In this case, we can consider the chance constraint on CLC term (and now it is a point-wise condition)
% %
% \begin{equation}\label{eq:CLF_QP_CCP}
% \begin{aligned}
% & \min_{\ubfu \in \underline{\calU}}\,\, \|L(\bfx)^\top(\ubfu - \underline{\tilde{\bfk}}(\bfx))\|^2 \\
% % \boldsymbol{u}^T H \boldsymbol{u} + p_d \delta^2 \\
% \mathrm{s.t.} \, \,  &\bbP(\textit{CLC}(\bfx,\ubfu) \leq 0) \geq 1- \beta. 
% \end{aligned}
% \end{equation}
% }

%link: https://bcci.me.berkeley.edu/downloads/papers/weehong_3.pdf

% Tan and Packard \cite{TanSearchingFC} proposed an approach to search for Control Lyapunov Functions (CLFs) using Sum of Squares (SOS) programming. Formally, consider a non-linear control-affine system:
% \begin{equation}\label{eq: dynamic}
% \begin{aligned}
%     \dot{\bfx} = f(\bfx) + g(\bfx) \bfu, 
% \end{aligned}
% \end{equation}
% %
% suppose that $f(\bf0) = 0$. A function $V$ is a Control Lyapunov Function (CLF) for this system if $V: \mathbb{R}^n \mapsto \mathbb{R}_{\geq 0}$ is a
% smooth, radially unbounded function such that: 
% \begin{equation}
% \label{eq: CLF_Origin}
%     \inf_{\bfu \in \mathbb{R}^m} \{ \frac{\partial V}{\partial \bfx} f(\bfx) + \frac{\partial V}{\partial \bfx} g(\bfx)\bfu\} < 0.
% \end{equation}
% Note that for any $\bfx \in \calX$ such that $\frac{\partial V}{\partial \bfx} g(\bfx) \neq 0$, one can make the inequality hold in \eqref{eq: CLF_Origin} by choosing a large value of $\bfu$ of the correct sign (requires no restriction on control space). Thus, the critical part is to satisfy the following condition:
% %
% \begin{equation}
%     \frac{\partial V}{\partial \bfx} f(\bfx) < 0 \; \; \forall \bfx \in \calX \; \text{such that} \; \frac{\partial V}{\partial \bfx} g(\bfx) = 0, \bfx \neq \bf0.
% \end{equation}
% If we restrict $f$ and $g$ be polynomial vector fields, we can use SOS programming to search for a valid polynomial CLF $V$.

% The problem now becomes: 
% \begin{align}
% \label{eq:origin_search}
%     &\text{find} \; V \in \calR_n \quad \quad \text{such that} \\
%     & V(\bfx) > 0 \; \forall \bfx \in \mathbb{R}^n \backslash \boldsymbol{0}, \; V(\boldsymbol{0}) = 0 \notag \\
%     & \Big\{ \bfx \in \mathbb{R}^n |  \frac{\partial V}{\partial \bfx} g(\bfx) = 0,   \frac{\partial V}{\partial \bfx} f(\bfx) \geq 0, \bfx \neq \bf0  \Big\} \text{is empty} \notag
% \end{align}

% \TODO{Based on the Positivstellensatz (P-satz), it is shown that the following SOS optimization program is a sufficient condition for problem \eqref{eq:origin_search} :} 
% %
% \begin{align}
% \label{eq: sos_clf}
%   &\min \gamma \quad \quad \text{over} \quad s_1 \in \Sigma_n,\; V,p_2 \in \calR_n \; \text{such that} \notag \\
%   & V- l_1 \in \Sigma_n; \notag \\
%   & -\Big\{ s_1 \left[ \frac{\partial V}{\partial \bfx} f(\bfx) - \gamma \right] + p_2 \left[\frac{\partial V}{\partial \bfx} g(\bfx) \right] \Big\} - l_2 \in \Sigma_n.
% \end{align}
% %
% where $\calR_n$ denotes the set of all polynomials of $n$ variables, $\Sigma_n$ denotes the set of sum of squares polynomials in $n$ variables, and $l_1, l_2$ are positive definite SOS polynomials. To ensure that \eqref{eq: sos_clf} has a chance of being satisfied, the polynomials we are searching over must satisfy the following degree conditions:
% %\KL{Why the degree conditions?}
% %
% \begin{align}
%     &\text{deg} V = \text{deg} l_1; \\
%     &\text{deg}(p_2Vg) \geq \text{deg} (s_1 V f); \\
%     &\text{deg} (p_2Vg) - 1 = \text{deg} l_2
% \end{align}
% %
% Note that the second constraint in \eqref{eq: sos_clf} is bi-linear (non-convex), the authors use iterative searching method to find the solution. 

% Furthermore, if we assume that the system is uncertain
% %
% \begin{equation}
%     \dot{\bfx} = f(\bfx)+g(\bfx)\bfu + d(\bfx)\bfomega, \; \bfomega \in \Omega
% \end{equation}
% %
% where
% %
% \begin{equation}
%     \Omega = \{ \bfomega \in \mathbb{R}^k: k_{\omega_i}(\bfomega) \geq 0, i = 1, \cdots, n_{\omega} \}
% \end{equation}
% %
% We can reformulate the SOS program in \eqref{eq: sos_clf} as follows: 
% %
% \begin{align}
%     &\min \gamma \quad \quad \text{over} \quad s_1 \in \Sigma_n,\; V,p_2 \in \calR_n \; \text{such that} \notag \\
%   & V-l_1 \in \Sigma_n; \notag \\
%   & -\Big\{ s_1 \left[ \frac{\partial V}{\partial \bfx} f(\bfx) - \gamma \right] + p_2 \left[\frac{\partial V}{\partial \bfx} g(\bfx) \right] +l_2  + \notag \\ &\sum_{i=1}^{n_\omega} \beta_i(\bfx,\omega) k_{\omega_i}(\omega)\Big\} \in \text{SOS}(\bfx,\omega); \notag \\
%   &\beta_i(\bfx,\omega) \in \text{SOS}(\bfx,\omega).
% \end{align}
% %
% where $l_1 = l_2 = \beta\|\bfx\|_2^2$. 



==> tex/CVaR_Lyapunov_Function.tex <==
\section{CVaR Lyapunov Function}
\label{sec: CVaR_Lyapunov_Function}
In the following, we take another perspective of enforcing stability of dynamic systems. 

We consider the uncertain dynamic system of the form (inspired by \cite{Ahmadi2020RiskSensitivePP})
%
\begin{equation}
\label{eq: Cvar_system}
    \bfx^{t+1} = f(\bfx^t, \bfu^t, \bfxi^t), \quad \bfx^{0} = \bfx_{0}.
\end{equation}
%
In \cite{Ahmadi2020RiskSensitivePP}, the authors propose the conditional-value-at-risk (CVaR) barrier functions for risk-averse controller synthesis using difference
convex programs (DCPs), under the assumption of stochastic linear discrete-time systems. Here, I try to generalize the idea to CVaR Lyapunov functions. 

Let's first assume a continuous differentiable function $V:
\bbR^n \mapsto \bbR_{\geq 0}$. In the following, we deal with the function $-\dot{V}(\bfx)$ and we want it to be non-negative with high probability.

\begin{lemma}[VaR and CVaR]
Given a confidence level $\beta \in (0,1)$, value-at-risk ($\text{VaR}_\beta$) denotes the $\beta$-quantile value of $-\dot{V}(\bfx)$ described as $\text{VaR}_\beta(-\dot{V}(\bfx)) = \sup_{\eta \in \bbR} \{\eta \; |\; \mathbb{P}( -\dot{V}(\bfx) \leq \beta \}$.

Conditional value-at-risk ($\text{CVaR}_\beta$) measures the expected value in the $\beta$-tail, that is $\text{CVaR}_\beta(-\dot{V}(\bfx)) = \mathbb{E} [-\dot{V}(\bfx) \; | \; -\dot{V}(\bfx) \leq \text{VaR}_\beta(-\dot{V}(\bfx))]$. $\text{CVaR}_\beta$ can also be given by an optimization formulation 
%
\begin{equation}
\label{eq: cvar_def}
    \text{CVaR}_\beta(-\dot{V}(\bfx)) := \inf_{\eta \in \bbR} \mathbb{E}\left[ \eta + \frac{(\dot{V}(\bfx) - \eta)_{+}}{\beta}   \right]
\end{equation}
%
\end{lemma}


\begin{definition}[CVaR Stability]
Given a confidence level $\beta \in (0,1)$, we call the solutions to \eqref{eq: Cvar_system} starting at $\bfx_0$ is CVaR-stable if and only if
%
\begin{equation}
\label{eq: cvar_stable}
    \text{CVaR}_{\beta}^{0:t} (-\dot{V}(\bfx^t)) < 0, \quad \forall t \geq 0.
\end{equation}
%
\TODO{The global stability is not guaranteed, but the stability along the trajectory is guaranteed with high probability.}
\end{definition}

In order to enforce the CVaR stability, we define CVaR Lyapunov functions. 

\begin{definition}[CVaR Lyapunov Function]
For the discrete-time system \eqref{eq: Cvar_system} and a confidence level $\beta \in (0,1)$, the continuous differentiable function $V:
\bbR^n \mapsto \bbR_{\geq 0}$ is a CVaR Lyapunov function, if there exists a constant $\alpha \in (0,1)$ such that
%
\begin{equation}
\label{eq: cvar_stable}
    \text{CVaR}_{\beta}^{t} (-\dot{V}(\bfx^{t+1})) \geq \alpha  (-\dot{V}(\bfx^{t})), \quad \forall \bfx^t \in \calX.
\end{equation}

\end{definition}
%
Similar to \cite{Ahmadi2020RiskSensitivePP}, one can demonstrate that the existence of a
CVaR Lyapunov function implies CVaR-stability. (\TODO{idea: using induction and the properties of coherent measure, one can show that if $-\dot{V}(\bfx^{0}) > 0$, then $-\dot{V}(\bfx^{t}) > 0$ for any $t > 0$. This implies that the system is $\text{CVaR}_\beta$-stable.}) 

\subsection{CVaR-Stable Controller Synthesis}

\TODO{In the following, assuming a valid nominal CLF $V(\bfx)$ is given for the system without uncertainty.}

At every time step $t$, given $\bfx^t$, a confidence
level $\beta \in (0, 1)$, a parameter $\alpha \in (0, 1)$, and a nominal controller $\tilde{\underline{\bfk}}(\bfx))$, solve

\begin{equation}
\label{eq: QP_origin}
\begin{aligned}
& \min_{\ubfu \in \underline{\calU}}\,\, \|L(\bfx)^\top(\ubfu - \tilde{\underline{\bfk}}(\bfx))\|^2\\
% \bfu^T H \bfu + p_d \delta^2 \\
\mathrm{s.t.} \, \,  &\text{CVaR}_{\beta}^{t} (\dot{V}( f(\bfx^t, \bfu^t, \bfxi^t))) \leq \alpha (\dot{V}(\bfx^{t}))
\end{aligned}
\end{equation}

==> tex/DR_CLF_SOS_.tex <==
\section{Distribuionally Robust CLF Search via Sum of Squares}
\label{sec: dr_sos_clf}

In this section, we extend the theory in Sec.~\ref{sec: approach_LF} to solve Problem.~\ref{prob: CLF_Construction}. Assume there is a polynomial nominal controller $\beta(\bfx)$, we now consider the distributionally robust CLF formulation as follows, 
%
\begin{equation}
\label{eq: drccp_clf_sos}
    \inf_{\mathbb{P}\in \calM_{N}^{r}}\bbP(-\dot{V}(\bfx,\bfxi) \geq 0  ) \geq 1-\alpha \; \forall \bfx \in \calX ,
\end{equation}
%
We first write down the expression for $\dot{V}(\bfx,\bfxi)$ with model uncertainty in \eqref{eq: uncertain_control_affine}. Using the kronecker product property $\text{vec}(\bfA\bfB\bfC) = (\bfC^\top \otimes \bfA)\text{vec}(\bfB)$ and the vectorization of $F(\bfx)$ in \eqref{eq: F_vectorization}, we have
%
\begin{align}
\label{eq: V_dot_control_affine}
    &\dot{V}(\bfx,\bfxi) = [\nabla_{\bfx} V(\bfx)]^\top F(\bfx)\beta(\bfx) + aV(\bfx) 
    = \beta(\bfx)^\top \text{vec}([\nabla_{\bfx} V(\bfx)]^\top F(\bfx)\bfI_{m+1}) + aV(\bfx) \notag \\
    &= \beta(\bfx)^\top(\bfI_{m+1} \otimes [\nabla_{\bfx} V(\bfx)]^\top)\text{vec}(F(\bfx)) + aV(\bfx) \notag \\
    & = \beta(\bfx)^\top \underbrace{(\bfI_{m+1} \otimes [\nabla_{\bfx} V(\bfx)]^\top)\text{vec}(\tilde{F}(\bfx))}_{q(\bfx)}+ aV(\bfx) + \beta(\bfx)^\top \underbrace{(\bfI_{m+1} \otimes [\nabla_{\bfx} V(\bfx)]^\top) \bfW(\bfx)}_{\bfR(\bfx)} \bfxi \notag \\
    & = \beta(\bfx)^\top q(\bfx) + \beta(\bfx)^\top \bfR(\bfx) \bfxi + aV(\bfx).
\end{align}
%
We now have the function $\dot{V}(\bfx, \bfxi)$ is affine in the uncertainty $\bfxi$. Following the same technique as in Proposition~\ref{proposition: drcc_sos}, we develop the distributionally robust chance constrained formulation of searching for a control Lyapunov function for the uncertain dynamical system \eqref{eq: uncertain_control_affine} as follows, 
%
%\begin{align}
%\label{eq: drccp_sos_clf_final}
%    &V(\bfx) = \sum_{i=1}^{d} c_i \bfx^i, \; c_0 = 0, \notag \\
%     &V(\bfx) - \epsilon\|\bfx\|_2^2 \in \text{SOS}(\bfx); \notag \\
%    - & r \beta(\bfx)^\top \bfR(\bfx)_j - \alpha(\dot{V}(\bfx,\bfxi_i) - \epsilon\|\bfx\|_2^2) \in \text{SOS}(\bfx), \notag \\
%    &r \beta(\bfx)^\top \bfR(\bfx)_j - \alpha(\dot{V}(\bfx,\bfxi_i) - \epsilon\|\bfx\|_2^2) \in \text{SOS}(\bfx), \notag \\
%    & \forall i = 1,2 \dots, N, \quad \forall j = 1,2 \dots, k. 
%\end{align}
%
%
\begin{align}
\label{eq: drccp_clf_constraint}
     &V(\bfx) \geq 0; \notag \\
    - & r \beta(\bfx)^\top \bfR(\bfx)_j - \alpha \dot{V}(\bfx,\bfxi_i) \geq 0, \notag \\
    &r \beta(\bfx)^\top \bfR(\bfx)_j - \alpha\dot{V}(\bfx,\bfxi_i)  \geq 0, \notag \\
    & \forall \bfx \in \calX, \quad \forall i = 1,2 \dots, N, \quad \forall j = 1,2 \dots, k. 
\end{align}

In the following, we aim at relaxing the assumption on known polynomial nominal controller $\beta(\bfx)$. We denote the nominal dynamics as $\tilde{f}(\bfx)$ and $\tilde{g}(\bfx)$. A CLF-QP to the nominal dynamics is: 
%
\begin{equation}
\begin{aligned}
\label{eq: clf_qp_nomi}
    &\min_{\bfu \in \calU} \| \bfu\|^2,  \\
    \mathrm{s.t.} \, \, &L_{\tilde{f}} V(\bfx) + L_{\tilde{g}} V(\bfx)\bfu + \alpha_V (V(\bfx)) \leq 0.
\end{aligned}
\end{equation}
%
Assume $V$ is a candidate CLF and  $L_{\tilde{g}} V(\bfx) = \mathbf{0}$ only if $L_{\tilde{f}} V(\bfx) + \alpha_V (V(\bfx)) < 0$. The closed-form solution to \eqref{eq: clf_qp_nomi} is given by:
\begin{equation} 
\label{sol: nomi_u}
	\tilde{\bfu} = \begin{cases}
	    -L_{\tilde{g}} V(\bfx)^{\top} \frac{L_{\tilde{f}} V(\bfx) + \alpha_V (V(\bfx))}{\| L_{\tilde{g}} V(\bfx) \|^2}, & L_{\tilde{f}} V(\bfx) + \alpha_V (V(\bfx)) \geq 0, \\
		\mathbf{0}, & L_{\tilde{f}} V(\bfx) + \alpha_V (V(\bfx)) < 0.
		\end{cases}\\
\end{equation}
%
First, we need to make sure that the CLF-QP subject to nominal system dynamics is feasible. Let $l_1, l_2$ be SOS polynomials, we need to ensure: 
%
\begin{align}
\label{cond: nomi_qp_feas}
    & V(\bfx) = \sum_{i=1}^{d} c_i \bfx^i, \ c_0 = 0, \quad \left\{ \bfx \in \calX | V(\bfx) \leq 0, l_1(\bfx) \neq 0 \right\} = \emptyset, \notag \\
    & \left\{\bfx \in \calX | L_{\tilde{g}} V(\bfx) = \mathbf{0}, L_{\tilde{f}} V(\bfx) + \alpha_V (V(\bfx)) \geq 0, l_2(\bfx) \neq 0 \right\} = \emptyset.
\end{align}
%
Our goal is to ensure that the CLF $V$ is distribuionally robust subject to the nominal controller given by \eqref{sol: nomi_u}. To achieve this, we need to satisfy \eqref{eq: drccp_clf_constraint} with $\beta(\bfx) := [1, \tilde{\bfu}^{\top}]^{\top}$. Note that for $L_{\tilde{f}} V(\bfx) + \alpha_V (V(\bfx)) \geq 0$, we have $\beta(\bfx)^{\top}q(\bfx) + a V(\bfx) = 0$. In this case, we just need to ensure the following set is empty,
%
\begin{equation}
\label{cond: dr_nz_u}
    \left\{ \bfx \in \calX | L_{\tilde{f}} V(\bfx) + \alpha_V (V(\bfx)) \geq 0, \alpha [1, \tilde{\bfu}^{\top}]\bfR(\bfx)(\bfxi_i \pm r \bfe_j)\geq 0, l_3(\bfx) \neq 0  \right\}
\end{equation}
%
for all $i = 1,2 \dots, N, \; \; j = 1,2 \dots, k$, where $l_3$ is an SOS polynomial and $\bfe_j \in \bbR^m$.

For the case $L_{\tilde{f}} V(\bfx) + \alpha_V (V(\bfx)) \leq 0$, we write $\beta(\bfx) := [1, \mathbf{0}_m^{\top}]^{\top}$ and need to ensure the following set is empty,
%
\begin{equation}
\label{cond: dr_z_u}
    \left\{ \bfx \in \calX | -L_{\tilde{f}} V(\bfx) - \alpha_V (V(\bfx)) \geq 0, \alpha  [1, \boldsymbol{0}_m^\top]\bfR(\bfx)(\bfxi_i \pm r \bfe_j) \geq 0, l_4(\bfx) \neq 0  \right\}
\end{equation}
%
for all $i = 1,2 \dots, N, \;\; j = 1,2 \dots, k$, where $l_4$ is an SOS polynomial and $\bfe_j \in \bbR^m$.
To ease notation, we write $\tilde{F}_V(\bfx) = L_{\tilde{f}} V(\bfx) + \alpha_V (V(\bfx))$. Applying P-satz to \eqref{cond: nomi_qp_feas}, we have the following SOS constraint \cite{TanSearchingFC}:
%
\begin{align}
\label{cond: nomi_qp_feas_sos}
    & V(\bfx) = \sum_{i=1}^{d} c_i \bfx^i, \ c_0 = 0; \; \; V(\bfx) - \epsilon\|\bfx\|_2^2 \in \text{SOS}(\bfx); \notag \\
    & -s_1\tilde{F}_V(\bfx) - L_{\tilde{g}} V(\bfx) \bfp_1 - l_2 
    \in \text{SOS}(\bfx),
\end{align}
%
where $\bfp_1$ is a vector of dimension $m$ with each element a polynomial of two variables and $s_1 \in \text{SOS}(\bfx)$. Similarly, we reformulate \eqref{cond: dr_nz_u} and \eqref{cond: dr_z_u} as the following SOS constraints:
%
\begin{equation}
\label{sos: dr_nz_u}
    -s_{2_{ij}} \tilde{F}_V(\bfx) - s_{3_{ij}} \alpha [1, \tilde{\bfu}^{\top}]\bfR(\bfx)(\bfxi_i \pm r \bfe_j) - l_3(\bfx) \in \text{SOS}(\bfx),
\end{equation}
%
%
\begin{equation}
\label{sos: dr_z_u}
    s_{4_{ij}} \tilde{F}_V(\bfx) - s_{5_{ij}} \alpha [1, \boldsymbol{0}_m^\top]\bfR(\bfx)(\bfxi_i \pm r \bfe_j) - l_4(\bfx) \in \text{SOS}(\bfx),
\end{equation}
%
for all $i = 1,2 \dots, N, \;\; j = 1,2 \dots, k$.
If we set $s_{2_{ij}} =  s_{3_{ij}} = \tilde{l}_3(\bfx)$, $s_{4_{ij}} =  s_{5_{ij}} = \tilde{l}_4(\bfx)$ for all $i,j$ and $l_3(\bfx) = \tilde{l}_3(\bfx)^2$, $l_4(\bfx) = \tilde{l}_4(\bfx)^2$, constraint \eqref{sos: dr_nz_u} and \eqref{sos: dr_z_u} would be reduced to:
%
\begin{equation}
\label{sos_simp: dr_nz_u}
    -\tilde{F}_V(\bfx) - \alpha [1, \tilde{\bfu}^{\top}]\bfR(\bfx)(\bfxi_i \pm r \bfe_j) - \tilde{l}_3(\bfx) \in \text{SOS}(\bfx),
\end{equation}
%
%
\begin{equation}
\label{sos_simp: dr_z_u}
    \tilde{F}_V(\bfx) - \alpha [1, \boldsymbol{0}_m^\top]\bfR(\bfx)(\bfxi_i \pm r \bfe_j) - \tilde{l}_4(\bfx) \in \text{SOS}(\bfx),
\end{equation}
%
for all $i = 1,2 \dots, N, \;\; j = 1,2 \dots, k$.
Expand $\bfR(\bfx)(\bfxi_i \pm r \bfe_j)$ as follows: $\bfR(\bfx)(\bfxi_i \pm r \bfe_j) = \nabla_{\bfx} V(\bfx)^\top( \hat{f}_{ij}^{\pm} + \hat{g}_{ij}^{\pm})$, we have $[1, \tilde{\bfu}^{\top}]\bfR(\bfx)(\bfxi_i \pm r \bfe_j) = \nabla_{\bfx} V(\bfx)^\top \hat{f}_{ij}^{\pm} + \frac{\nabla_{\bfx} V(\bfx)^\top \hat{g}_{ij}^{\pm} \tilde{g}^{\top}\nabla_{\bfx} V(\bfx)}{\nabla_{\bfx} V(\bfx)^\top \tilde{g} \tilde{g}^{\top}\nabla_{\bfx} V(\bfx)}$. If $g$ is known, we have equation above reduced to: $[1, \tilde{\bfu}^{\top}]\bfR(\bfx)(\bfxi_i \pm r \bfe_j) = \nabla_{\bfx} V(\bfx)^\top \hat{f}_{ij}^{\pm} + k_{ij}^{\pm}$ with $k_{ij}^{\pm}$ equals to the sum of all elements of its corresponding $(\bfxi_i \pm r \bfe_j)$.
%\TODO{Problem: $[1, \tilde{\bfu}^{\top}]^{\top}$ is a function of $V$ and $\bfR(\bfx)$ is a function of $V$ as well, causing non-linearity in decision variables.}
%\left\{ \bfx \in \calX | -L_{\tilde{f}} V(\bfx) - \alpha_V (V(\bfx)) \geq 0, \alpha  [1, \mathbf{0}_m^{\top}]\bfR(\bfx)\bfxi_i + \alpha (L_{\tilde{f}} V(\bfx) + \alpha_V (V(\bfx))) \pm r  [1, \mathbf{0}_m^{\top}]\bfR(\bfx)_j \geq 0, l_4(\bfx) \neq 0  \right\}

==> tex/DR_SOS.tex <==
\section{Distributional Robust Control Lyapunov Function Search}
\label{sec: approach}

\subsection{Asymptotic Global Stability}
Given the observation samples of $f,g$ (\TODO{How do we collect samples of $f,g$ given the state-control sequence dataset (e.g. online GP regression)?}), we can compute the empirical distribution of $f,g$ as $\hat{\mathbb{P}}_{N}(f)$ and $\hat{\mathbb{P}}_{N}(g)$, respectvely.

% \KL{Maybe we should consider  $\hat{\mathbb{P}}_{N}(F)$ directly?}.

we present an approach of searching a valid CLF for uncertain system dynamics with only $\hat{\mathbb{P}}_{N}(f)$ and $\hat{\mathbb{P}}_{N}(g)$ available.  

In the following, we consider $\Xi$ to be a complete separable
metric space with metric $d$. Let $\calB(\Xi)$ and $\calP(\Xi)$ be the Borel
$\sigma$-algebra and the set of Borel probability measures on $\Xi$. First, we define the data-driven Wasserstein ambiguity set around $\hat{\mathbb{P}}_{N}(f)$ and $\hat{\mathbb{P}}_{N}(g)$: 
%
\begin{align}
      &\calM_{N}^{r_1} := \{\mu \in \calP_p(\Xi) | W_p(\mu,\hat{\mathbb{P}}_{N}(f) ) \leq r_1\},   \\
      &\calM_{N}^{r_2} := \{\mu \in \calP_p(\Xi) | W_p(\mu,\hat{\mathbb{P}}_{N}(g) ) \leq r_2\},  
\end{align}
%
where $\calP_p(\Xi) \subset \calP(\Xi)$ is the set of Borel probability measures
with finite $p$-th moment for $p \in [1, \infty)$.

\TODO{In the neural Lyapunov function setting, how do we apply DRO with the $\max$ symbol in the loss function? In Sec.\ref{sec: RCLBF}, the authors ensure the robustness by considering all $f$ and $g$ in the loss function and sum them together.}


\subsection{Distributional Robust Formulation of Neural Lyapunov Function}






==> tex/Evaluation_Yi.tex <==
\section{Evaluation}
We demonstrate that the proposed methods to find stable Lyapunov functions on various nonlinear dynamical systems and find candidate control Lyapunov functions on complex non-linear robot control problems. 

\subsection{Lyapunov Function Search}
In the following, we consider the following dynamical system: 
%
\begin{equation}\label{eq: case_1_dynamic}
\begin{aligned}
    \underbrace{\dot{\left[ \begin{matrix}
    x_1 \\
    x_2 
    \end{matrix} \right]}}_{\dot{\bfx}}
	=	
	\underbrace{\left[ \begin{matrix}
			-\frac{3}{2}x_1^3 - \frac{1}{2}x_1^2 - x_2  \\
			6x_1 - x_2
			\end{matrix} \right]}_{f(\bfx)}
\end{aligned}
\end{equation}
%
We assume the system above is uncertain with the following parametric uncertainty:
%
\begin{equation}
\label{eq: case_1_uncert}
    \dot{\bfx} = f(\bfx) + \sum_{i = 1}^n d(\bfx)_i\xi_i
\end{equation}
%
where $d(\bfx)_i \in \bbR^2, \xi_i \in \bbR$ for all $i \in [n]$.
In the following, we compare the SOS search results with polynomial degree $d = 4$ for the orginal formulation \eqref{eq: original_lf_sos}, chance constrained formulation \eqref{eq: ccp_sos_final}, and distributionally robust chance constrained formulation \eqref{eq: drccp_sos_final}. We use $3$ offline uncertainty samples $\{ \bfxi_i \}_{i = 1}^{3}$ and set the confidence level $\alpha = 0.3$ for all the cases that are listed below.
\\
%\textit{Case 1 (Degree 1 Single Perturbation):} $r = 0.03, \ n = 1, \ d(\bfx) = [0,-x_2]^{\top}, \ \bfxi_i \in (2:0.25:4), \ \bfxi^* = 4.3$. \\
\textit{Case 1 (Degree 1 Double Perturbation):} $r = 0.6, \ n = 2, \ d(\bfx)_1 = [-x_1,-x_2]^{\top}, \ d(\bfx)_2 = [-x_2,0]^{\top}, \ \bfxi_i \in [\{2.5,3,3.5\},\{2.5\}]^{\top}, \ \bfxi^* = [1.5,4.6]^{\top}$. \\
\textit{Case 2 (Degree 3 Double Perturbation):} $r = 0.45, \ n = 2, \ d(\bfx)_1 = [-(x_1^3+x_2),-x_2]^{\top}, \ d(\bfx)_2 = [-x_2,-x_1]^{\top}, \ \bfxi_i \in [\{2.5,3,3.5\},\{2.5\}]^{\top}, \ \bfxi^* = [1.1,3.8]^{\top}$. \\
%The Results are shown in the following figures:
%
\setcounter{subfigure}{0}
%\begin{figure}[t]
%	\centering
%	\subfigure[Case 1 with Original SOS Search]{\includegraphics[width=.3\linewidth]{fig/SOS_case1.eps}\label{fig: case_1_sos}}
%	\subfigure[Case 1 with CCP-SOS Search]{\includegraphics[width=.3\linewidth]{fig/CCP_case1.eps}\label{fig: case_1_ccp}}
%	\subfigure[Case 1 with DRCCP-SOS Search]{\includegraphics[width=.3\linewidth]{fig/DRCCP_case1.eps}\label{fig: case_1_drccp}}
%	\caption{Red area indicates $\dot{V} > 0$.}
%\end{figure}
%
\begin{figure}[t]
	\centering
	\subfigure[Case 1 with Original SOS Search Violation rate: $33.96 \% $; $\dot{V}_{\text{max}} = 2033$.]{\includegraphics[width=.3\linewidth]{fig/SOS_case2.eps}\label{fig: case_1_sos}}
	\subfigure[Case 1 with CCP-SOS Search Violation rate: $8.10 \% $; $\dot{V}_{\text{max}} = 57.8$.]{\includegraphics[width=.3\linewidth]{fig/CCP_case2.eps}\label{fig: case_1_ccp}}
	\subfigure[Case 1 with DRCCP-SOS Search Violation rate: $0 \% $; $\dot{V}_{\text{max}} = 0$.]{\includegraphics[width=.3\linewidth]{fig/DRCCP_case2.eps}\label{fig: case_1_drccp}}
	%\caption{Red area indicates $\dot{V} > 0$.}
    \vfill
    \subfigure[Case 2 with Original SOS Search. Violation rate: $35.85 \% $; $\dot{V}_{\text{max}} = 694.5$.]{\includegraphics[width=.3\linewidth]{fig/SOS_case4.eps}\label{fig: case_2_sos}}
	\subfigure[Case 2 with CCP-SOS Search. Violation rate: $8.57 \% $; $\dot{V}_{\text{max}} = 18.77$.]{\includegraphics[width=.3\linewidth]{fig/CCP_case4.eps}\label{fig: case_2_ccp}}
	\subfigure[Case 2 with DRCCP-SOS Search. Violation rate: $0 \% $; $\dot{V}_{\text{max}} = 0$.]{\includegraphics[width=.3\linewidth]{fig/DRCCP_case4.eps}\label{fig: case_2_drccp}}
	\caption{Red area indicates $\dot{V} > 0$.}
\end{figure}
%
%\begin{figure}[t]
%	\centering
%	\subfigure[Case 3 with Original SOS Search. Violation rate: $21.3 \% $; $\dot{V}_{\text{max}} = 6800$.]{\includegraphics[width=.3\linewidth]{fig/SOS_case3.eps}\label{fig: case_3_sos}}
%	\subfigure[Case 3 with CCP-SOS Search. Violation rate: $0.05 \% $; $\dot{V}_{\text{max}} = 0.035$.]{\includegraphics[width=.3\linewidth]{fig/CCP_case3.eps}\label{fig: case_3_ccp}}
%	\subfigure[Case 3 with DRCCP-SOS Search. Violation rate: $0 \% $; $\dot{V}_{\text{max}} = 0$.]{\includegraphics[width=.3\linewidth]{fig/DRCCP_case3.eps}\label{fig: case_3_drccp}}
%	\caption{Red area indicates $\dot{V} > 0$.}
%\end{figure}
%

==> tex/Related_work.tex <==
\section{Related Work}
\label{sec: related_work}

%ref: https://ocw.mit.edu/courses/16-s498-risk-aware-and-robust-nonlinear-planning-fall-2019/cf42518d50e9f3a686718eac2d8515e8_MIT16_S498f19_L14.pdf

If uncertainty appears in the system dynamics 
%
\begin{equation}
\label{eq: uncertain_system}
    \dot{\bfx} = f(\bfx, \bfomega) = f(\bfx) + d(\bfx)\bfxi
\end{equation}
%
where $\bfx \in \calX \subseteq \mathbb{R}^{n}$ is the robot state and $\bfxi \in \Xi = \{ \bfxi \in \mathbb{R}^k: g_{\xi_i}(\bfxi) \geq 0, i = 1, \cdots, k \}$ is the uncertainty. 

One can formulate the following program to search for a valid Lyapunov function for the uncertain system \eqref{eq: uncertain_system}. 
%
\begin{align}
\label{eq: robust_sos}
     &V(\bfx) = \sum_{i=1}^{d} c_i \bfx^i, \notag \\
     &V(\bfx) - \epsilon\|\bfx\|_2^2 \in \text{SOS}(\bfx); \notag \\
     &-\dot{V}(\bfx,\bfxi) - \epsilon\|\bfx\|_2^2 - \notag \sum_{i=1}^{k} \alpha_i(\bfx,\bfxi) g_{\xi_i}(\bfxi) \in \text{SOS}(\bfx,\bfxi); \notag \\
   &\alpha_i(\bfx,\bfxi) \in \text{SOS}(\bfx,\bfxi).
\end{align}
%
% \KL{We may replace $\alpha_i(\bfx,\bfxi)$ as a scalar $c_i^2$, as long as the nonnegativity is assured.}

\subsection{Case Study I}
In the following, we consider the following uncertain system: 
%
\begin{equation}\label{eq: case_1_system}
\begin{aligned}
    \underbrace{\dot{\left[ \begin{matrix}
    x_1 \\
    x_2 
    \end{matrix} \right]}}_{\dot{\bfx}}
	=	
	\underbrace{\left[ \begin{matrix}
			-\frac{3}{2}x_1^3 - \frac{1}{2}x_1^2 - x_2  \\
			6x_1
			\end{matrix} \right]}_{f(\bfx)}
	+
	\underbrace{\left[ \begin{matrix}
		0 & 0\\
		-x_2 & 0
		\end{matrix} \right]}_{d(\bfx)}\left[\begin{matrix}
    \xi_1 \\
    \xi_2 
    \end{matrix} \right]
\end{aligned}
\end{equation}
%
where $\xi_1 \in [3,5]$ and $\xi_2 = 0$. The following result is solved with polynomial degree $ d = 4$. 

% \KL{If the range of $\xi$ is $[-1,1]$, the program seems infeasible. Also, if the sign of $\xi$ changes, the program does not work as well. What are the restrictions/properties of $d(\bfx)$?}

\begin{figure}[t]
\centering
\subcaptionbox{$\xi_1 = 3$ \label{fig:1a}}{\includegraphics[width=0.33\linewidth]{fig/case1_w=3.png}}%
\hfill%
\subcaptionbox{$\xi_1 = 5$ \label{fig:1b}}{\includegraphics[width=0.33\linewidth]{fig/case1_w=5.png}}%
\hfill%
\subcaptionbox{$\xi_1 = 0$ \label{fig:1c}}{\includegraphics[width=0.33\linewidth]{fig/case1_w=0.png}}%
\label{fig:case1_result}
\vspace*{-3ex}
\end{figure}


\subsection{Case Study II}
In the following, we consider the following uncertain system: 
%
\begin{equation}\label{eq: case_1_system}
\begin{aligned}
    \underbrace{\dot{\left[ \begin{matrix}
    x_1 \\
    x_2 
    \end{matrix} \right]}}_{\dot{\bfx}}
	=	
	\underbrace{\left[ \begin{matrix}
			-\frac{3}{2}x_1^3 - \frac{1}{2}x_1^2 - x_2  \\
			6x_1
			\end{matrix} \right]}_{f(\bfx)}
	+
	\underbrace{\left[ \begin{matrix}
		-x_1 & -x_2\\
		-x_2 & 0
		\end{matrix} \right]}_{d(\bfx)}\left[\begin{matrix}
    \xi_1 \\
    \xi_2 
    \end{matrix} \right]
\end{aligned}
\end{equation}
%
where $\xi_1 \in [3,5]$ and $\xi_2 \in [1,3]$.

\begin{figure}[t]
\centering
\subcaptionbox{$\xi_1 = 3,\xi_2 = 2 $ \label{fig:2a}}{\includegraphics[width=0.33\linewidth]{fig/case2_w1=3_w2=2.png}}%
\hfill%
\subcaptionbox{$\xi_1 = 1, \xi_2 = 3$ \label{fig:2b}}{\includegraphics[width=0.33\linewidth]{fig/case2_w1=1_w2=3.png}}%
\hfill%
\subcaptionbox{$\xi_1 = 3, \xi_2 = 8$ \label{fig:2c}}{\includegraphics[width=0.33\linewidth]{fig/case2_w1=3_w2=8.png}}%
\label{fig:case2_result}
\vspace*{-3ex}
\end{figure}

% \KL{In the experiment, if the degree in $d(\bfx)$ is greater than $1$, the SOS becomes infeasible. }
